DomainVerse: A Benchmark Towards Real-World Distribution Shifts For Tuning-Free Adaptive Domain Generalization

Traditional cross-domain tasks, including domain adaptation and domain generalization, rely heavily on training model by source domain data. With the recent advance of vision-language models (VLMs), viewed as natural source models, the cross-domain task changes to directly adapt the pre-trained source model to arbitrary target domains equipped with prior domain knowledge, and we name this task Adaptive Domain Generalization (ADG). However, current cross-domain datasets have many limitations, such as unrealistic domains, unclear domain definitions, and the inability to fine-grained domain decomposition, which drives us to establish a novel dataset DomainVerse for ADG. Benefiting from the introduced hierarchical definition of domain shifts, DomainVerse consists of about 0.5 million images from 390 fine-grained realistic domains. With the help of the constructed DomainVerse and VLMs, we propose two methods called Domain CLIP and Domain++ CLIP for tuning-free adaptive domain generalization. Extensive and comprehensive experiments demonstrate the significance of the dataset and the effectiveness of the proposed methods.

==> table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|ccccc|ccc|cc|ccc|ccc|ccccc}
\toprule
& & & \multicolumn{5}{c}{Weather} & \multicolumn{3}{c}{View} & \multicolumn{2}{c}{Time} & \multicolumn{3}{c}{Scene} & \multicolumn{3}{c}{Season} &\multicolumn{5}{c}{Occlusion} \\
& Method & Average & C & SA & F & R & SN & F & L & T & D & N & F & H & M & S & A & W & UN & L & P & M & H \\
\multirow{3}{*}{Zero-shot} & Zero-shot CLIP & 36.41 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
& \textbf{CALIP} & \textbf{39.67} & \textbf{40.98} & \textbf{34.03} & 41.22 & 40.77 & 44.70 & 40.37 & 58.32 & 20.32 & 42.82 & 36.52 & 43.18 & 36.38 & 39.44    & 37.40 & 40.78 & 40.60 & 51.05 & 33.95 & 39.93 & 38.52 & 34.91 \\
& CLIP+DN & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\multirow{4}{*}{Name-only} & VisDesc  & 36.45 & 37.76 & 31.11 & 38.07 & 37.14 & 41.67 & 37.32 & 54.30 & 17.74 & 40.08 & 32.82 & 39.42 & 33.90 & 36.04 & 34.16 & 37.46 & 37.48 & 47.83 & 30.87 & 36.40 & 35.49 & 31.68 \\
& CuPL & 36.24 & 37.56 & 30.91 & 38.06 & 36.61 & 41.74 & 36.50 & 54.30 & 17.93 & 39.73 & 32.76 & 38.45 & 34.14 & 36.14 & 33.62 & 37.30 & 37.49 & 47.31 & 30.80 & 36.12 & 35.43 & 31.55 \\
& CuPL+e & 37.48 & 38.78 & 31.98 & 39.30 & 38.14 & 42.65 & 38.14 & 55.43 & 18.88 & 40.77 & 34.20 & 40.46 & 34.65 & 37.34 & 35.07 & 38.56 & 38.55 & 48.93 & 31.85 & 37.51 & 36.65 & 32.48 \\
& SuS-X & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
Test-time-adaptation & TPT & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\multirow{2}{*}{Ours} & Domain CLIP & 40.58 & 42.31 & 34.20 & 42.60 & 42.16 & 43.73 & 40.63 & 60.85 & 20.26 & 43.43 & 37.73 & 45.22 & 36.70 & 39.82 & - & 41.97 & 40.82 & - & - & - & - & - \\
& Domain++ CLIP& 40.36 & 41.89 & 34.50 & 42.21 & 41.45 & 44.55 & 40.59 & 60.78 & 19.71 & 43.05 & 37.67 & 44.83 & 36.97 & 39.28 & 38.42 & 41.46  & 41.03  & - & - & - & - & -  \\ \bottomrule
\end{tabular}}
\end{table*}
